Softmax Bias Correction for Quantized Generative Models

Post-training quantization (PTQ) is the go-to compression technique for large generative models, such as stable diffusion or large language models. PTQ methods commonly keep the softmax activation in higher precision as it has been shown to be very sensitive to quantization noise. However, this can lead to a significant runtime and power overhead during inference on resource-constraint edge devices. In this work, we investigate the source of the softmax sensitivity to quantization and show that the quantization operation leads to a large bias in the softmax output, causing accuracy degradation. To overcome this issue, we propose an offline bias correction technique that improves the quantizability of softmax without additional compute during deployment, as it can be readily absorbed into the quantization parameters. We demonstrate the effectiveness of our method on stable diffusion v1.5 and 125M-size OPT language model, achieving significant accuracy improvement for 8-bit quantized softmax.

==> idf_boxes.tex <==
Q1. Name your Invention.
Softmax Bias Correction in quantized diffusion models

Q2.Describe the problem or situation being addressed that led to your solution.
Background: As Quantized Aware Training (QAT) methods are not practically feasible for large generative models due to training data and resource constraints, PTQ methods are go to methods for on-device deployment. Unet of stable diffusion model is very sensitive to lower precisions, hence making it difficult to quantize the network to INT8 or lower.

Problem: Softmax output in unet of stable diffusion is biased and causes loss of softmax attention (output of softmax) and hence affects the model’s performance when quantized to lower bits. This prevents PTQ from achieving an optimum quantized solution.

Known literatures on quantization of diffusion models keep softmax layers in higher (INT16/FP16) or full precision while enabling PTQ based solutions.


Q3.Describe the invention including any known technical advantages or benefits.
(a) We propose a statistical technique to correct the biased nature of the softmax output. Our method improves the quantizability of the sensitive softmaxes present in the Unet network helping in achieving a better lower precision PTQ based quantized network for deployment.

(b) Our proposed method is based on offline correction and has no additional latency overhead during deployment. Our method also improves the visual quality of the quantized generated image and makes the images more closer to full precision output.



Q4. How could we determine if someone is using this invention?

If we have access to the code. 




